Data-Efficient Molecular Generation with Hierarchical Textual Inversion

Developing an effective molecular generation framework even with a limited number of molecules is often important for its practical deployment, e.g., drug discovery, since acquiring task-related molecular data requires expensive and time-consuming experimental costs. To tackle this issue, we introduce Hierarchical textual Inversion for Molecular generation (HI-Mol), a novel data-efficient molecular generation method. HI-Mol is inspired by the importance of hierarchical information, e.g., both coarse- and fine-grained features, in understanding the molecule distribution. We propose to use multi-level embeddings to reflect such hierarchical features based on the adoption of the recent textual inversion technique in the visual domain, which achieves data-efficient image generation. Compared to the conventional textual inversion method in the image domain using a single-level token embedding, our multi-level token embeddings allow the model to effectively learn the underlying low-shot molecule distribution. We then generate molecules based on the interpolation of the multi-level token embeddings. Extensive experiments demonstrate the superiority of HI-Mol with notable data-efficiency. For instance, on QM9, HI-Mol outperforms the prior state-of-the-art method with 50x less training data. We also show the effectiveness of molecules generated by HI-Mol in low-shot molecular property prediction.

==> figures/optimization_figure.tex <==
% \begin{figure*}[t]
% \centering\small
% \vspace{-0.1in}
% \includegraphics[width=0.5\textwidth]{NeurIPS2023/figures/himol_optimization.pdf}
% \vspace{-0.1in}
% \caption{
% Visualizations of the molecules for generated in PlogP conditional generation experiments. The maximum PlogP value among the training molecules is 4.52; \sjline{[sj]revising}.
% }
% \label{fig:optimization}
% \vspace{-0.2in}
% \end{figure*}


\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.18in}
\includegraphics[width=\linewidth]{NeurIPS2023/figures/himol_optimization.pdf} 
\vspace{-0.25in}

\caption{Visualization of the generated molecules with condition $\gamma$. The maximum PLogP among the training molecules is 4.52.}
\label{fig:conditional_generation}
%\vspace{-0.1in}
\end{wrapfigure}

